Improved Photometric Redshifts with Surface Luminosity Priors

We apply Bayesian statistics with prior probabilities of galaxy surface luminosity (SL) to improve photometric redshifts. We apply the method to a sample of 1266 galaxies with spectroscopic redshifts in the GOODS North and South fields at 0.1 < z < 2.0. We start with spectrophotometric redshifts (SPZs) based on Probing Evolution and Reionization Spectroscopically grism spectra, which cover a wavelength range of 6000-9000A, combined with (U)BViz(JHK) broadband photometry in the GOODS fields. The accuracy of SPZ redshifts is estimated to be \sigma (\Delta(z))=0.035 with an systematic offset of -0.026, where \Delta(z)=\Delta z / (1+z), for galaxies in redshift range of 0.5 < z < 1.25. The addition of the SL prior probability helps break the degeneracy of SPZ redshifts between low redshift 4000 A break galaxies and high-redshift Lyman break galaxies which are mostly catastrophic outliers. For the 1138 galaxies at z < 1.6, the fraction of galaxies with redshift deviation \Delta (z) > 0.2 is reduced from 15.0% to 10.4%, while the rms scatter of the fractional redshift error does not change much.

==> Revision <==
Main points we made changes:

1. Figure 4 updated with the profiles fitting parameters changed in both figure, caption and text, the changes are marked in black font.

2. Figure 5 and 6 are updated with labels 'SB' changed to 'SL'.

3. All citation in paper to "Cohen et al. (2008)" are changed to "Cohen et al. (2009, in prep)"

4. In page 3, we add citation to "Hathi et al. (2008)" when we define the surface luminosity priors in unit of luminosity per area.

5. In page 6 the first paragraph, when we first mention the elliptical galaxies, we add citation to "Ferreras et al. (2009), submitted", where we obtained the sample.

6. In page 6 the equation (2), we correct the frequency "\nu_B" to frequency interval "\Delta\nu_B".

7. We update the numbers of our sample and the calculation. The changes are all minor changes in number, like "1199" to "1266", "277" to "283", "0.034" to "0.035", etc., they are marked in black font in the text. 

